Gravitational wave populations and cosmology with neural posterior estimation

We apply neural posterior estimation for fast-and-accurate hierarchical Bayesian inference of gravitational wave populations. We use a normalizing flow to estimate directly the population hyper-parameters from a collection of individual source observations. This approach provides complete freedom in event representation, automatic inclusion of selection effects, and (in contrast to likelihood estimation) without the need for stochastic samplers to obtain posterior samples. Since the number of events may be unknown when the network is trained, we split into sub-population analyses that we later recombine; this allows for fast sequential analyses as additional events are observed. We demonstrate our method on a toy problem of dark siren cosmology, and show that inference takes just a few minutes and scales to $\sim 600$ events before performance degrades. We argue that neural posterior estimation therefore represents a promising avenue for population inference with large numbers of events.

==> schemata/schema_classical_method_nf.tex <==


\begin{figure}
    \centering
    \begin{tikzpicture}[
    squarednode/.style={rectangle, draw=black!60, fill=blue!5, very thick, minimum size=10mm, scale = 0.75}, 
    % square with arrows
    pics/rr/.style={code={
    \draw[] (0,0) -- (0.2,0) -- (0.2,0.2) -- (0.0,0.2) -- cycle;
    \draw[->] (0.1,-0.1) -- (0.1,-0.5) ;
    }},
    % only arrows
    pics/rrarrow/.style={code={
    \draw[->] (0.1,0.3) -- (0.1,-0.5) ;
    }},
    ]
    \node[squarednode,align=center]      (ps)  {\large GW data};
    \node[squarednode,align=center, yshift = -1cm, xshift = 1.0cm] (clasbilby) [below left =of ps] {Single-event posterior\\ estimation, e.g.~\bilby};
    \node[squarednode,align=center] (claspopu) [below =of clasbilby] {Population posterior \\estimation, e.g.~\icarogw};
     %%%%%%%%%%%%%%%%%
     \coordinate[above=of clasbilby] (B) ;
     \coordinate[below=of claspopu] (C) ;
     \coordinate (V) at ( $ (C)!0.5!(B) $ );
     %%%%%%%%%%%%%%%%%
     \node[squarednode,xshift=-3.7cm,align=center, draw=red!60, fill=red!5] (FL) at (V) {Classical \\ inference};
     \draw[red,thick,dashed] ($(clasbilby.north west)+(-0.6,0.6)$)  rectangle ($(claspopu.south east)+(0.6,-0.6)$);
     %%%%%%%%%%%%%%%%%
     \draw[->] (ps.west) -- (clasbilby.north |- ps.west) -- (clasbilby.north);
    \draw[->] (clasbilby.south) -- (claspopu.north) node [pos=0.5,right,font=\footnotesize]  {};
    %%%%%%%%%%%%%%%%%
    % ML part
    %%%%%%%%%%%%%%%%%
    \node[squarednode,align=center, xshift = -1.0cm] (dingo) [below right =of ps] {Single-event posterior\\estimation, e.g.~DINGO};
    \node[squarednode,align=center] (ourmodel) [below =of dingo] {Population posterior \\estimation, our model};
    \node[squarednode,align=center] (combine) [below =of ourmodel] {Combine sub-posteriors via\\importance sampling};
    % some code, the shape rr is defined above
    \path foreach \X in {0,1,...,8}
 { ($(dingo.south)+(0.3 * \X - 1.3, -0.4)$) pic{rr}};
    %%%%%%%%%%%%%%%%%
    % some code, the shape rrarrow is defined above
    \path foreach \X in {0,1,...,8}
 { ($(ourmodel.south)+(0.3 * \X - 1.3, -0.4)$) pic{rrarrow}};
    %%%%%%%%%%%%%%%%%
    \coordinate (V2) at ( $ (dingo)!0.5!(combine) $ );
     \node[squarednode,xshift=4.6cm,align=center, draw=cyan!60, fill=cyan!5] (FL) at (V2) {Likelihood-free \\inference};
     \draw[cyan,thick,dashed] ($(dingo.north west)+(-0.6,0.6)$)  rectangle ($(combine.south east)+(0.6,-0.6)$);
     %%%%%%%%%%%%%%%%%
     \draw[->] (ps.east) -- (dingo.north |- ps.east) -- (dingo.north);
    \end{tikzpicture}
    \caption{Comparison between the classical method and our model. Small white squares indicate batches of events (containing a subset of GW events). We split the problem of population inference analyzing many events in multiple simpler problems analyzing a subset of all events in the catalog. We then combine the resulting distributions a posteriori to obtain the full posterior distribution. }
    \label{methods: machine learning: schema comparison classical lf inference}
\end{figure}

==> schemata/summary_embedding_networks.tex <==

\begin{landscape}
\begin{figure}
    \centering
    \begin{tikzpicture}[
    squarednode/.style={rectangle, draw=black!60, fill=blue!5, very thick, minimum size=10mm, scale = 1},
    % square with arrows
    pics/rr/.style={code={
    \draw[] (0,0) -- (0.2,0) -- (0.2,0.2) -- (0.0,0.2) -- cycle;
    \node[inner sep=0pt] (corner) at (0,0) {\includegraphics[width=2.7cm]{schemata/corner_plot_example_GW150914_low.pdf}};
    \draw[->] (1.8,0) -- (2.8,0);
    \node[squarednode,align=center, draw=red!60, fill=magenta!5] at (4.2,0) {Embedding\\network 1};
    \draw[->] (5.6,0) -- (6.6,0);
    }},]
    % define GW data
    \node[rectangle,
        draw = lightgray,
        text = black,
        fill = magenta!3,
        minimum width = 1.6cm, 
        minimum height = 10cm,
        align = center] (r) at (-11.3, 4.5) {GW\\catalog};
    % add opening brace
    \draw [decorate,thick, decoration = {calligraphic brace, mirror}] (-10.45,7.) --  (-10.45,8.5);
    % define opening shape
    \draw[xshift = 0.1 cm] (-10.4,7) -- (-10.4,8.5) -- (-8.3,10.5) -- (-8.3, -1.5) -- cycle ;
    % some code, the shape rr is defined above
    \path foreach \X in {0,2,3}
 { ($(0,0)+(-6.0, 3 * \X)$) pic{rr}};
    % Calligraphic brace
    \draw [decorate,thick,
    decoration = {calligraphic brace}] (-8,-1.5) --  (-8,10.5);
    \node[align=center] (punktpunkt) at (-6,3) {\large $\ldots$}; 
    \node[align=center] (input) at (-9.3,7.75) {Input data:\\$\nbatchevents$ events};
    % order of magnitude comments
    \node[yshift = 7.cm] (x) [above =of punktpunkt]{$\nbatchevents\times\npost \times 3$};
    \node[align=center] (orderofmagn) at (x-|input) {Information\\content};
    \node[align=center, xshift = 4.2cm] (embinformation) at (x) {$\nbatchevents\times\mathcal{O}(16)$};
    % #####
    % define the embedding network 2
    \node[rectangle,
        draw = lightgray,
        text = olive,
        fill = green!3,
        minimum width = 1cm, 
        minimum height = 10cm,
        align = center] (emb2) at (2, 4.5) {Embedding\\network 2};
    % information content embedding network 2
    \node[align=center] (embinformation2) at (x-|emb2) {$\mathcal{O}(128)$};
    % add rectangle around information content
    \draw[thick,dashed,draw = blue] ($(orderofmagn.north west)+(-0.3,+0.3)$) rectangle ($(embinformation2.south east)+(0.3,-0.5)$);
    % #####
    \node[align=center] at (4,5) {Condition\\-ing};
    \draw[->] (3.5,4.5) -- (4.5,4.5);
    % #####
    \node[rectangle,
    draw = lightgray,
    text = blue,
    fill = blue!3,
    minimum width = 1cm, 
    minimum height = 2cm,
    align = center] (nflow) at (6, 4.5) {Normalizing\\flow};
    % #####
    \draw[->] (6,7) -- (6,6);
    \draw[->] (6,3) -- (6,2);
    % ##### define coordinates
    \coordinate (nflowZplotcoord) at (6,8.5);
    \coordinate (nflowYplotcoord) at (6,0.5);
    % #####
    \node[inner sep=0pt] (nflowZplot) at (nflowZplotcoord) {\includegraphics[width=3cm]{schemata/example_normal_Z.png}};
    \node[inner sep=0pt] (nflowYplot) at (nflowYplotcoord) {\includegraphics[width=3.cm]{schemata/example_normal_Y.png}};
    % #####
    \end{tikzpicture}
    \caption{Overview of the data reduction with the embedding networks and the conditioning of the normalizing flow. This method reduces the data dimension from initially $\nbatchevents\times\npost\times 3$ to $\mathcal{O}(128)$. This data summary significantly simplifies the training process of the network.  }
    \label{ml results: fig: our method and embedding networks}
\end{figure}

\end{landscape}
